Algorithmic Complexity of Power Law Networks

It was experimentally observed that the majority of real-world networks follow power law degree distribution. The aim of this paper is to study the algorithmic complexity of such "typical" networks. The contribution of this work is twofold. First, we define a deterministic condition for checking whether a graph has a power law degree distribution and experimentally validate it on real-world networks. This definition allows us to derive interesting properties of power law networks. We observe that for exponents of the degree distribution in the range $[1,2]$ such networks exhibit double power law phenomenon that was observed for several real-world networks. Our observation indicates that this phenomenon could be explained by just pure graph theoretical properties. The second aim of our work is to give a novel theoretical explanation why many algorithms run faster on real-world data than what is predicted by algorithmic worst-case analysis. We show how to exploit the power law degree distribution to design faster algorithms for a number of classical P-time problems including transitive closure, maximum matching, determinant, PageRank and matrix inverse. Moreover, we deal with the problems of counting triangles and finding maximum clique. Previously, it has been only shown that these problems can be solved very efficiently on power law graphs when these graphs are random, e.g., drawn at random from some distribution. However, it is unclear how to relate such a theoretical analysis to real-world graphs, which are fixed. Instead of that, we show that the randomness assumption can be replaced with a simple condition on the degrees of adjacent vertices, which can be used to obtain similar results. As a result, in some range of power law exponents, we are able to solve the maximum clique problem in polynomial time, although in general power law networks the problem is NP-complete.

==> mathdots.tex <==
%%
%% This is file `mathdots.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% mathdots.dtx  (with options: `tex')
%% 
%% -------------------------------------------------------------------
%% 
%% Copyright 2001--2014, Daniel H. Luecking
%% 
%% Mathdots may be distributed and/or modified under the conditions of the
%% LaTeX Project Public License, either version 1.3 of this license or (at
%% your option) any later version. The latest version of this license is in
%%    <http://www.latex-project.org/lppl.txt>
%% and version 1.3 or later is part of all distributions of LaTeX version
%% 2003/12/01 or later.
%% 
%% Mathdots has maintenance status "author-maintained". The Current
%% Maintainer is Daniel H. Luecking. The Base Interpreters associated with
%% mathdots are plain TeX and LaTeX
%% 
\def\mathdotsfiledate{2014/06/11}%
\def\mathdotsfileversion{0.9}%
\expandafter
\ifx\csname MathDots\mathdotsfileversion\endcsname\relax
\else
  \immediate\write16{Mathdots already loaded.}\expandafter\endinput
\fi
\immediate\write16{Package mathdots, \mathdotsfiledate\space version
  \mathdotsfileversion.}%
\expandafter\edef\csname MathDots\mathdotsfileversion\endcsname{%
    \catcode`\noexpand\@=\the\catcode`@}%
\catcode`\@=11
\def\@nameuse#1{\csname#1\endcsname}%
\def\MDo@us#1{\@nameuse{#1style}}%
\def\MDo@uf#1{\@nameuse{#1font}0}%
\def\MDo@t{text}\def\MDo@s{script}\def\MDo@ss{scriptscript}%
\newdimen\MDo@unit \MDo@unit\p@
\def\MDo@changestyle#1{\relax\MDo@unit0.1\fontdimen6\MDo@uf{#1}%
  \everymath\expandafter{\the\everymath\MDo@us{#1}}}%
\def\MDo@dot{$\m@th\ldotp$}%
\def\MDo@palette#1{\mathchoice{#1\MDo@t}{#1\MDo@t}{#1\MDo@s}{#1\MDo@ss}}%
\def\MDo@ddots#1{{\MDo@changestyle{#1}%
  \mkern1mu\raise7\MDo@unit\vbox{\kern7\MDo@unit\hbox{\MDo@dot}}%
  \mkern2mu\raise4\MDo@unit\hbox{\MDo@dot}%
  \mkern2mu\raise \MDo@unit\hbox{\MDo@dot}\mkern1mu}}%
\def\MDo@vdots#1{\vbox{\MDo@changestyle{#1}%
  \baselineskip4\MDo@unit\lineskiplimit\z@
  \kern6\MDo@unit\hbox{\MDo@dot}\hbox{\MDo@dot}\hbox{\MDo@dot}}}%
\def\MDo@iddots#1{{\MDo@changestyle{#1}%
  \mkern1mu\raise \MDo@unit\hbox{\MDo@dot}%
  \mkern2mu\raise4\MDo@unit\hbox{\MDo@dot}%
  \mkern2mu\raise7\MDo@unit\vbox{\kern7\MDo@unit\hbox{\MDo@dot}}}}%
\def\fixedvdots{%
  \vbox{\baselineskip4\p@ \lineskiplimit\z@
  \kern6\p@\hbox{.}\hbox{.}\hbox{.}}}%
\def\fixedddots{%
  \mathinner{\mkern1mu
  \raise7\p@\vbox{\kern7\p@\hbox{.}}\mkern2mu
  \raise4\p@\hbox{.}\mkern2mu
  \raise\p@\hbox{.}\mkern1mu}}%
\def\fixediddots{%
  \mathinner{\mkern1mu
  \raise\p@\hbox{.}\mkern2mu
  \raise4\p@\hbox{.}\mkern2mu
  \raise7\p@\vbox{\kern7\p@\hbox{.}}\mkern1mu}}%
\let\originalddots=\ddots
\let\originalvdots=\vdots
\let\originaliddots=\iddots
\def\MDoddots{%
  \mathinner{\MDo@palette\MDo@ddots}}%
\def\MDoiddots{%
  \mathinner{\MDo@palette\MDo@iddots}}%
\def\MDovdots{%
  \mathinner{\MDo@palette\MDo@vdots}}%
\wlog{Mathdots Info: Redefining \string\ddots.}%
\wlog{Mathdots Info: Redefining \string\vdots.}%
\let\ddots \MDoddots
\let\iddots\MDoiddots
\let\vdots \MDovdots
\newbox\MDo@dotsbox
\newmuskip\MDoprekern
\newmuskip\MDopostkern
\newmuskip\MDodotkern
\MDoprekern 0mu
\MDopostkern -1mu
\MDodotkern -1.3 mu
\def\MDo@dotsaccent#1{\mathpalette{\MDo@@dotsaccent{#1}}}%
\let\originaldddot \dddot
\let\originalddddot\ddddot
\def\MDo@@dotsaccent#1#2#3{%
{%
  \setbox\MDo@dotsbox\hbox{$#2\mkern\MDoprekern#1\mkern\MDopostkern$}%
  \mathop{#3\kern\z@}\limits^{\text{\ex@.2326ex
    \vbox to-1.4\ex@{\kern-1.8\ex@\copy\MDo@dotsbox\vss}}}%
}}%
\ifx\amstexloaded@\relax % true if amstex has been loaded
  % A backup test in case \amstexloaded@ became \relax by accident:
  \ifx\ddddot\UndEfInEd
  \else
    \def\MDo@D{\mathchar"5F\mkern\MDodotkern}%
    \wlog{Mathdots Info: Redefining \string\dddot.}%
    \wlog{Mathdots Info: Redefining \string\ddddot.}%
    \def\MDodddot {\MDo@dotsaccent{\MDo@D\MDo@D\MDo@D}}%
    \def\MDoddddot{\MDo@dotsaccent{\MDo@D\MDo@D\MDo@D\MDo@D}}%
    \let\dddot \MDodddot
    \let\ddddot\MDoddddot
  \fi
\fi
\csname MathDots\mathdotsfileversion\endcsname
\endinput
%%
%% End of file `mathdots.tex'.

